An Interleaved Approach to Trait-Based Task Allocation and Scheduling

To realize effective heterogeneous multi-robot teams, researchers must leverage individual robots' relative strengths and coordinate their individual behaviors. Specifically, heterogeneous multi-robot systems must answer three important questions: \textit{who} (task allocation), \textit{when} (scheduling), and \textit{how} (motion planning). While specific variants of each of these problems are known to be NP-Hard, their interdependence only exacerbates the challenges involved in solving them together. In this paper, we present a novel framework that interleaves task allocation, scheduling, and motion planning. We introduce a search-based approach for trait-based time-extended task allocation named Incremental Task Allocation Graph Search (ITAGS). In contrast to approaches that solve the three problems in sequence, ITAGS's interleaved approach enables efficient search for allocations while simultaneously satisfying scheduling constraints and accounting for the time taken to execute motion plans. To enable effective interleaving, we develop a convex combination of two search heuristics that optimizes the satisfaction of task requirements as well as the makespan of the associated schedule. We demonstrate the efficacy of ITAGS using detailed ablation studies and comparisons against two state-of-the-art algorithms in a simulated emergency response domain.

==> sections/0_preamble.tex <==
\IEEEoverridecommandlockouts % This command is only needed if 
   % you want to use the \thanks command

\overrideIEEEmargins % Needed to meet printer requirements.

% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document
%related research
%clear vision of contribution
%what experiments/sim to expect
%logical flow

% The following packages can be found on http:\\www.ctan.org
\usepackage{caption}
\usepackage{subcaption}
\usepackage{epsfig} % for postscript graphics files
\usepackage{times} % assumes new font selection scheme installed
\usepackage{subcaption}
%\usepackage{fixltx2e}
\usepackage{svg}
\usepackage{tabu}
\usepackage[utf8]{inputenc}

    \RequirePackage{mathbbol}
    \newcommand{\hmmax}{0}
    \newcommand{\bmmax}{2}
\usepackage{bm}
%\usepackage[allowlitunits]{siunitx}
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\usepackage{booktabs,tabu}
\usepackage{diagbox}

% Alter some LaTeX defaults for better treatment of figures:
% See p.105 of "TeX Unbound" for suggested values.
% See pp. 199-200 of Lamport's "LaTeX" book for details.
%   General parameters, for ALL pages:
\renewcommand{\topfraction}{0.9}	% max fraction of floats at top
\renewcommand{\bottomfraction}{0.8}	% max fraction of floats at bottom
%   Parameters for TEXT pages (not float pages):
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}     % 2 may work better
\setcounter{dbltopnumber}{2}    % for 2-column pages
\renewcommand{\dbltopfraction}{0.9}	% fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}	% allow minimal text w. figs
%   Parameters for FLOAT pages (not text pages):    \renewcommand{\floatpagefraction}{0.7}	% require fuller float pages
% N.B.: floatpagefraction MUST be less than topfraction !!
\renewcommand{\dblfloatpagefraction}{0.7}	% require fuller float pages
% remember to use [htp] or [htpb] for placement

%Math Stuff
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bbm} %to support numbers in mathbb
\usepackage{amsfonts}

\usepackage{moreverb}
\usepackage{url}
\usepackage{hyperref} % Cross-referencing
\usepackage{cleveref} % More cross-referencing. MUST BE AFTER hyperref
% \usepackage{amsthm} % Various enhancements for defining theorem-like structures
\usepackage{graphicx} % Importing/manipulating graphics
\usepackage{listings} % Psuedocode
\usepackage{xcolor}
\usepackage{cite}
\usepackage{ifthen}

% Pseudocode Stuff
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}


%Table Stuff
\usepackage{array} %for table entries to be in center of cell
\usepackage{tabularx}
\usepackage{multicol}
\usepackage{multirow}
 \usepackage{zref-xr}

% Setup images folder
\graphicspath{ {./images/} }

%=======U S E R  D E F I N E D  M A C R O S=======
\newcommand{\todo}[1]{\textcolor{red}{[#1]}}
\newcommand{\edit}[1]{\textcolor{blue}{#1}}
\newcommand{\cut}[1]{\textcolor{red}{#1}}
\newcommand{\tocite}[0]{\textcolor{red}{[cite]}}
\newcommand{\etal}[0]{et al.}

% Custom Math Operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Var}{Var}

% Custom Aliases for Symbols
\newcommand{\R}{\ensuremath{\mathbb{R}}} % Real Numbers
\newcommand{\N}{\ensuremath{\mathbb{N}}} % Natural Numbers
\newcommand{\Q}{\ensuremath{\mathbb{Q}}} % Rationals
\newcommand{\Z}{\ensuremath{\mathbb{Z}}} % Integers
\newcommand{\C}{\ensuremath{\mathbb{C}}} % Complex
\newcommand{\eps}{\ensuremath{\varepsilon}} % epsilon
\newcommand{\grad}{\ensuremath{\nabla}} % Gradient
\newcommand{\defeq}{\ensuremath{::=}} % Definition equals
\newcommand{\bigo}{\ensuremath{\mathcal{O}}} % Big O

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}

% Usage:
% \subseclabel{mysection} creates \label{subsec:mysection}
% \subsecref{mysection} references it
\newcommand{\subseclabel}[1]{\label{subsec:#1}}
\newcommand{\subsecref}[1]{Subsection~\ref{subsec:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

%% Circled number
%% http://tex.stackexchange.com/questions/7032/good-way-to-make-textcircled-numbers
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=0.7pt] (char) {\footnotesize{#1}};}}

%% Surround with:
%%% parentheses
\newcommand{\parens}[1]{\left(#1\right)}
%%% brackets
\newcommand{\brackets}[1]{\left\{#1\right\}}
%%% angled brackets
\newcommand{\angled}[1]{\left\langle#1\right\rangle}
%%% square brackets
\newcommand{\sqBrackets}[1]{\left[#1\right]}
%%% open open interval
\newcommand{\ooint}[1]{\parens{#1}}
%%% closed closed interval
\newcommand{\ccint}[1]{\sqBrackets{#1}}
%%% closed open interval
\newcommand{\coint}[1]{\left\[#1\right)}
%%% open closed interval
\newcommand{\ocint}[1]{\left(#1\right]}
%%% floor
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
%%% ceiling
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
%%% rephrase
\newcommand{\rephrase}[1]{\color{red}#1\color{black}}

\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{property}{Property}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

% Punctuation in math environment
\ifdefined\comma 
	\renewcommand{\comma}{\ensuremath{\, \text{, }}}
\else 
	\newcommand{\comma}{\ensuremath{\, \text{, }}}
\fi
\newcommand{\semicolon}{\ensuremath{\, \text{; }}}
\newcommand{\fullstop}{\ensuremath{\, \text{. }}}

\newenvironment{flushitemize}{%
	\begin{list}{$\bullet$}
		{\setlength{\leftmargin}{20pt}}%
		\setlength{\labelwidth}{20pt}
		\setlength{\itemindent}{0pt}
		\setlength{\labelsep}{0.5em}
		\setlength{\itemsep}{1pt}
		\setlength{\parskip}{0pt}
		\setlength{\parsep}{0pt}}
	{\end{list}}


\setlength{\textfloatsep}{5pt}
\setlength{\intextsep}{5pt}
\setlength{\dbltextfloatsep}{5pt}
\setlength{\dblfloatsep}{5pt}

% Pseudocode
\let\oldnl\nl
\newcommand{\nolinenumber}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\newcommand{\customcomment}[1]{\nolinenumber // #1}



==> sections/10_acknowledgements.tex <==
\section{ACKNOWLEDGMENT}
This work was supported by the Army Research Lab under Grant W911NF-17-2-0181 (DCIST CRA). 

==> sections/6_comparison.tex <==


\section{Comparison to Existing ST-MR-TA Algorithms}



==> sections/9_FutureWork.tex <==
\section{Future Work}
In the experimentation used to validate our method's performance, a lazy PRM was used for motion planning. This algorithm, while simple and potentially fast, is unable to consider robot collisions. More advanced motion planners may be more suitable for teams of heterogeneous robots. Adding a more robust and advanced motion planner would increase our method's ability to deal with the intricacies of multi-robot teams.

%Additionally, our method used a tabu search to select the orderings for disjunctive constraints. This proved to be the slowest part of our method, and another type of search or methodology could improve performance. In the future, we hope to examine several other methodologies for selecting the orderings of disjunctive constraints and get a better understanding of their strengths and weaknesses.

Finally, the present approach takes a task network as input. In the future, we hope to pair this method with a task planner capable of generating this task network. This combined approach would further increase the capabilities of teams of robots who use our approach.

==> sections/comparision_chart.tex <==
\begin{table*}[!tb]
    \centering
    \begin{tabular}{|cccccccc|}
        \hline
        {Algorithm}                                                   &{Agent/Task}         &{Assignment}         &{Heterogeneous}    &{Temporal}              &{Hard}             &{Require All}         &{Motion}\\
        {}                                                            &{Modeling}           &{Constraints}        &{Agents}           &{Constraints}           &{Constraints}      &{Tasks Be Completed}   &{Planning}\\   
        \hline
        ITAGS(Ours)                                                   &Continuous Traits    &\checkmark           &\checkmark         &Ordering                &\checkmark         &\checkmark            &Continuous\\
        \hline
        Capezzuto et al.(2020)\cite{Capezzuto2020}                          &Utility              &                     &\checkmark         &Deadline                &\checkmark         &                      &Discrete\\
        \hline
        Kabir et al.(2020)\cite{Kabir2020IncorporatingManipulators}         &Utility              &                     &                   &Ordering                &\checkmark         &\checkmark            &Continuous\\
        \hline
        Thakar et al.(2019)\cite{Thakar2019TaskManipulation}                &Utility              &                     &                   &Ordering/Deadline        &\checkmark        &\checkmark            &Continuous\\
        \hline 
        Parker et al.(2016)\cite{Parker2016ExploitingTeamwork}              &Utility              &\checkmark           &\checkmark         &Deadline                &                   &                      &\\
        \hline
        Pujol-Gonzalez et al.(2015)\cite{Pujol-Gonzalez2015}                &Utility              &                     &                   &Ordering/Deadline       &\checkmark         &                      &\\
        \hline
        Giordani et al.(2013)\cite{Giordani2013}                           &Utility              &                     &                   &None                     &                  &                       &\\
        \hline
        Korsah et al.(2012)\cite{Korsah2012}              &Utility              &                     &                   &Ordering/Deadline       &\checkmark         &\checkmark            &\\
        \hline
        Jones et al.(2011)\cite{Jones2011Time-extendedConstraints}          &Utility              &\checkmark           &\checkmark         &Ordering                &\checkmark         &                      &Discrete\\
        \hline
        Sariel et al.(2006)\cite{Sariel2006}                                &Utility              &                     &\checkmark         &Ordering                &\checkmark         &\checkmark            &\\
        \hline
        Koes et al.(2006)\cite{Koes2006ConstraintRobotics}                  &Binary Traits        &\checkmark           &\checkmark         &Complex                 &\checkmark         &                      &\\
        \hline
        Tompkins et al.(2003)\cite{Tompkins2003OptimizationOperations}      &Utility              &\checkmark           &\checkmark          &Ordering                &\checkmark         &\checkmark            &\\
        \hline
        Shehory and Kraus(1998)\cite{Shehory1998MethodsFormation}           &Utility              &                     &                   &Ordering                &\checkmark         &\checkmark            &\\
        \hline
        %Krizmancic et al.\cite{Krizmancic2020}                        &Utility              &\checkmark           &\checkmark          &Ordering                &\checkmark        &\checkmark            &\\
        %\hline
        %Koes et al.\cite{Koes2005HeterogeneousConstraints}            &Binary Traits        &\checkmark           &\checkmark         &Deadline                &                   &                      &Discrete\\
        %\hline
        %Amador et al.(2014)\cite{Amador2014}                               &Utility              &                     &  %\hline
        %\hline       
        % Guerro et al.\cite{Guerrero2017Multi-robotSolutions}        &Utility              &                     &                   &None                     &                  &\checkmark            &\\
        %\hline
        
    \end{tabular}
    \caption{Comparison of Existing ST-MR-TA Algorithms}
    \tablabel{comp}
\end{table*}



==> sections/comparision_old.tex <==

\begin{table*}[!tbh]
    \centering
    \begin{tabular}{|c|cccccccccccc|}
        \hline
        {Algorithm}     &\rotatebox[origin=c]{90}{ITAGS}     &\rotatebox[origin=c]{90}{Capezzuto et al.\cite{Capezzuto2020}}  &\rotatebox[origin=c]{90}{Su et al.\cite{Su2016CoordinationConstraints}  } &\rotatebox[origin=c]{90}{Parker et al.\cite{Parker2016ExploitingTeamwork}} &\rotatebox[origin=c]{90}{Pujol-Gonzalez et al.\cite{Pujol-Gonzalez2015EfficientRescue}}  &\rotatebox[origin=c]{90}{Amador et al.\cite{Amador2014DynamicConstraints}} &\rotatebox[origin=c]{90}{Korsah et al.\cite{Korsah2012XBots:Dependencies}   } &\rotatebox[origin=c]{90}{Jones et al.\cite{Jones2011Time-extendedConstraints}} &\rotatebox[origin=c]{90}{Sariel et al.\cite{Sariel2006}} &\rotatebox[origin=c]{90}{Koes et al.\cite{Koes2006ConstraintRobotics}} &\rotatebox[origin=c]{90}{Koes et al.\cite{Koes2005}} &\rotatebox[origin=c]{90}{Shehory and Kraus\cite{Shehory1998MethodsFormation} }\\ 
        \hline
        {Agent/Task}  &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark    &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark  &\checkmark\\
        {Modeling}  & & & & & & & & & & & &\\
        \hline
        {Assignment}   &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark    &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark\\
        {Constraints} & & & & & & & & & & & &\\
        \hline
        {Heterogeneous}     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark    &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark\\
        {Agents} & & & & & & & & & & & &\\
        \hline
        {Temporal}  &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark    &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark\\
        {Constraints}  & & & & & & & & & & & &\\
        \hline
        {Hard}  &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark    &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark\\
        {Constraints} & & & & & & & & & & & &\\
        \hline
        {Requires All Tasks} &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark    &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark\\
        {Be Completion}  & & & & & & & & & & & &\\
        \hline
        {Motion} &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark    &\checkmark     &\checkmark     &\checkmark     &\checkmark     &\checkmark\\
        {Planning}  & & & & & & & & & & & &\\
        \hline
    \end{tabular}
    \caption{Comparison of Existing ST-MR-TA Algorithms}
    \tablabel{comp}
\end{table*}



\begin{table*}[!tbh]
    \centering
    \begin{tabular}{|cccccccc|}
        \hline
        {Algorithm}                                                   &{Agent/Task}         &{Assignment}         &{Heterogeneous}    &{Temporal}              &{Hard}             &{Require All}         &{Motion}\\
        {}                                                            &{Modeling}           &{Constraints}        &{Agents}           &{Constraints}           &{Constraints}      &{Task Be Completed}   &{Planning}\\   
        \hline
        \hline
        ITAGS(Ours)                                                   &Continuous Traits    &\checkmark           &\checkmark         &Ordering                &\checkmark         &\checkmark            &Continuous\\
        \hline
        Capezzuto et al.\cite{Capezzuto2020}                          &Utility              &                     &\checkmark         &Deadline                &\checkmark         &                      &Discrete\\
        \hline
        Su et al.\cite{Su2016CoordinationConstraints}                 &Utility              &                     &\checkmark         &Deadline                &\checkmark         &                      &\\
        \hline
        Parker et al.\cite{Parker2016ExploitingTeamwork}              &Utility              &\checkmark           &\checkmark         &Deadline                &                   &                      &\\
        \hline
        Pujol-Gonzalez et al.\cite{Pujol-Gonzalez2015EfficientRescue} &Utility              &                     &                   &Ordering/Deadline       &\checkmark         &                      &\\
        \hline
        Amador et al.\cite{Amador2014DynamicConstraints}              &Utility              &                     &                   &Deadline                &                   &\checkmark            &\\
        \hline
        Korsah et al.\cite{Korsah2012XBots:Dependencies}              &Utility              &                     &                   &Ordering/Deadline       &\checkmark         &\checkmark            &\\
        \hline
        Jones et al.\cite{Jones2011Time-extendedConstraints}          &Utility              &\checkmark           &\checkmark         &Ordering                &\checkmark         &                      &Discrete\\
        \hline
        Sariel et al.\cite{Sariel2006}                                &Utility              &                     &\checkmark         &Ordering                &\checkmark         &\checkmark            &\\
        \hline
        Koes et al.\cite{Koes2006ConstraintRobotics}                  &Binary Traits        &\checkmark           &\checkmark         &Complex                 &\checkmark         &                      &\\
        \hline
        Koes et al.\cite{Koes2005}                                    &Binary Traits        &\checkmark           &\checkmark         &Deadline                &                   &                      &Discrete\\
        \hline
        Shehory and Kraus\cite{Shehory1998MethodsFormation}           &Utility              &                     &                   &Ordering                &\checkmark         &\checkmark            &\\
        \hline
    \end{tabular}
    \caption{Comparison of Existing ST-MR-TA Algorithms}
    \tablabel{comp}
\end{table*}



